A Graph Neural Network Approach to Automated Model Building in Cryo-EM Maps

Electron cryo-microscopy (cryo-EM) produces three-dimensional (3D) maps of the electrostatic potential of biological macromolecules, including proteins. Along with knowledge about the imaged molecules, cryo-EM maps allow de novo atomic modelling, which is typically done through a laborious manual process. Taking inspiration from recent advances in machine learning applications to protein structure prediction, we propose a graph neural network (GNN) approach for automated model building of proteins in cryo-EM maps. The GNN acts on a graph with nodes assigned to individual amino acids and edges representing the protein chain. Combining information from the voxel-based cryo-EM data, the amino acid sequence data and prior knowledge about protein geometries, the GNN refines the geometry of the protein chain and classifies the amino acids for each of its nodes. Application to 28 test cases shows that our approach outperforms the state-of-the-art and approximates manual building for cryo-EM maps with resolutions better than 3.5 \r{A}.

==> introduction.tex <==
\section{Introduction}

    Following rapid developments in microscopy hardware and image processing software, cryo-EM structure determination of biological macromolecules is now possible to atomic resolution for favourable samples \citep{nakane2020single, yip2020atomic}. For many other samples, such as large multi-component complexes and membrane proteins, resolutions around 3 \r{A} are typical \citep{cheng2018single}. Transmission electron microscopy images are taken of many copies of the same molecules, which are frozen in a thin layer of vitreous ice. Dedicated software, like RELION \citep{scheres2012relion} or cryoSPARC \citep{punjani2017cryosparc}, implement iterative optimization algorithms to retrieve the orientation of each molecule and perform 3D reconstruction to obtain a voxel-based map of the underlying molecular structure. 
    
    Provided the cryo-EM map is of sufficient resolution, it is interpreted in terms of an atomic model of the corresponding molecules. Many samples contain only proteins; other samples also contain other biological molecules, like lipids or nucleic acids. Proteins are linear chains of amino acids or residues. There are twenty different canonical amino acids that make up proteins. All of these amino acids have four heavy (non-hydrogen) atoms that make up the protein's main chain. The different amino acids have different numbers, types, and geometrical arrangements of their side-chain atoms. The smallest amino acid, glycine, has no heavy side chain atoms; the largest amino acid, tryptophan, has ten heavy side chain atoms. Typical proteins range in size from tens to more than a thousand residues. Typically, the electron microscopist knows which protein sequences are present in the sample. The task at hand is to build the atomic model, which identifies the positions of all atoms for all proteins that are present in the cryo-EM map. For each residue, there are two rotational degrees of freedom in the conformation of its main chain, the $\Phi$ and $\Psi$ angles. Distinct orientations of the side chains provide additional conformational possibilities, the number of which depends on the type of amino acid (figure \hyperref[fig:naming]{1}). 
    
    \begin{figure}[]
            \label{fig:naming}
            \centering
            \includegraphics[width=\textwidth]{figures/naming.png}
            \caption{\textbf{(A)} shows a peptide backbone where the chain is ordered from left to right. Arrows mark the peptide bonds between the C atom of one residue and the N atom of the next. \textbf{(B)} shows six amino acids, pointing out the differences in the side chains, marked by the outline. \textbf{(C)} shows the $\Phi$ and $\Psi$ angles of the backbone and the additional rotatable bond of the side chain for threonine.}
        \end{figure}
        
    Atomic model building in cryo-EM maps is typically done manually using 3D visualisation software, \citep[e.g.][]{coot,pettersen2021ucsf}, followed by refinement procedures that optimize the fit of the models in the map, \citep[e.g.][]{murshudov2011refmac5, isolde, phenix}. 
    Often, in areas of weak density in the map, one cannot discern the amino acid identity of residues from the map alone and sequence information has to be used to make an accurate assessment.
    Manually building a reliable atomic model \emph{de novo} in the reconstructed cryo-EM map is considered to be difficult for maps with resolutions worse than 4 \r{A}. Although the task is more straightforward for maps with resolutions better than 3 \r{A}, it still typically requires large amounts of time and a high level of expertise. 
    
    Machine learning has recently achieved a major step forward in structure prediction for individual proteins \citep{jumper2021highly, baek2021accurate}.
    In these approaches, the sequence information of proteins and their evolutionary related homologues is used to predict their atomic structure without the use of experimental data.
    In addition, protein language models, which are trained in an unsupervised fashion on the amino acid sequences of many proteins, have also provided useful results in protein structure prediction \citep{lin2022esmfold, wu2022omegafold}. 
    Although these techniques are not yet capable of reliably predicting structures of the larger complexes that are typically studied by cryo-EM, their success for individual proteins inspired us to explore similar approaches for automated model building in cryo-EM maps. 
    
    In this paper, we present a single integrated GNN that combines the voxel-based information from the cryo-EM map with information from the protein sequence through a protein language model, and information from the topology of the graph through invariant point attention (IPA) \citep{jumper2021highly}. For 28 test cases, we demonstrate that our approach approximates the accuracy of manual model building for maps with resolutions better than 3.5 \r{A}. 
    



==> methods.tex <==
\section{Methods}

    \input{paper_tex_files/methods_tex_files/residue_segmentation.tex}

    \input{paper_tex_files/methods_tex_files/all_atom_refinement.tex}
    
    \input{paper_tex_files/methods_tex_files/postprocessing.tex}


==> paper_tex_files/discussion_tex_files/next_steps.tex <==
\subsection{Next steps}
    There are a few missing features in ModelAngelo that we aim to add in the future. The first priority is to develop a model that does not need amino-acid sequences as an input and can, instead, help biologists by sequencing cryo-EM densities through searches in large databases like Uniclust \cite{mirdita2017uniclust}. The second priority is support for nucleotides, which the pipeline currently lacks. The main barrier for this is to properly define the torsion angles and the representative coordinate frames. Lastly, we can leverage the development of powerful protein structure predictors like AlphaFold2 by using the structures built by our model as templates to fit predicted structures. Using these template-based approaches could allow for automatically building models in maps of lower resolution, which we aim to investigate in the future. 


